Users really do respond to smishing

Text phish messages, referred to as Smishing is a type of social engineering attack where fake text messages are created, and used to lure users into responding to those messages. These messages aim to obtain user credentials, install malware on the phones, or launch smishing attacks. They ask users to reply to their message, click on a URL that redirects them to a phishing website, or call the provided number. Thousands of mobile users are affected by smishing attacks daily. Drawing inspiration by the works of Tu et al. (USENIX Security, 2019) on Robocalls and Tischer et al. (IEEE Symposium on Security and Privacy, 2016) on USB drives, this paper investigates why smishing works. Accordingly, we designed smishing experiments and sent phishing SMSes to 265 users to measure the efficacy of smishing attacks. We sent eight fake text messages to participants and recorded their CLICK, REPLY, and CALL responses along with their feedback in a post-test survey. Our results reveal that 16.92% of our participants had potentially fallen for our smishing attack. To test repeat phishing, we subjected a set of randomly selected participants to a second round of smishing attacks with a different message than the one they received in the first round. As a result, we observed that 12.82% potentially fell for the attack again. Using logistic regression, we observed that a combination of user REPLY and CLICK actions increased the odds that a user would respond to our smishing message when compared to CLICK. Additionally, we found a similar statistically significant increase when comparing Facebook and Walmart entity scenario to our IRS baseline.

==> surveyresponse.tex <==
\section{Survey Responses}
In this section, we provided the recorded responses for the post experiment survey. We received 2 survey responses in Qualtrics, 12 voice call, but 9 were either silent or no useful information. We only had 3 meaningful feedback. In text reply, we got 21 but few of them are blanks or funny memes, we got 5 meaningful survey mentioned in the table. For for all click experiments, we have got total 44 clicks, however, we only got 1 response for E1 and 1 response for E12. 

Most of the survey respondents were aware about the scam but still they responded. In the SMS phishing context, any responses is valuable to hackers. The persons who convinced about the phishing mentioned that due to the local number, important government information and tax lawsuit convinced them to fall into the phishing. As per PhishMe~\cite{phishme} 2017, curiosity is one of the top motivator of phishing attacks. 

\begin{table*}[]
\centering
\begin{tabular}{|l|l|l|l|}
\hline
\multicolumn{1}{|c|}{\textbf{No.}} & Action & \multicolumn{1}{c|}{\textbf{Reasons for respond}} & Aware? \\ \hline
E1 & CLICK & Curiosity. & Yes \\ \hline
\multirow{2}{*}{E2} & \multirow{2}{*}{REPLY} & Because we do not spend that kind of money at any Walmart & Yes \\ \cline{3-4} 
 &  & Credit card fraud & Yes \\ \hline
\multirow{3}{*}{E5} & \multirow{3}{*}{CALL} & \begin{tabular}[c]{@{}l@{}}The fact that the area code for the phone number was the city of my school. So it made it \\ like more realistic, rather than a random area code from a different city-state or country.\end{tabular} & No \\ \cline{3-4} 
 &  & \begin{tabular}[c]{@{}l@{}}Important government information, just because it has to do with taxes, it has to do with \\ security numbers and all kinds of personal information.\end{tabular} & No \\ \cline{3-4} 
 &  & The fact that you were threatening me about my tax information. & No \\ \hline
\multirow{2}{*}{E7} & \multirow{2}{*}{REPLY} & If this is legit where do you get your contact list from? & Yes \\ \cline{3-4} 
 &  & Wow, you cock smokers are persistent. You can represent these nuts for free. & Yes \\ \hline
E12 & CLICK & \begin{tabular}[c]{@{}l@{}}I often find them funny, so I still open them even if I know it's fake. Also helps \\ me educate myself on how these cons work.\end{tabular} & Yes \\ \hline
\end{tabular}
\caption{Summary of valid survey responses}
\end{table*}






